A Framework for Empowering Reinforcement Learning Agents with Causal Analysis: Enhancing Automated Cryptocurrency Trading

Despite advances in artificial intelligence-enhanced trading methods, developing a profitable automated trading system remains challenging in the rapidly evolving cryptocurrency market. This research focuses on developing a reinforcement learning (RL) framework to tackle the complexities of trading five prominent altcoins: Binance Coin, Ethereum, Litecoin, Ripple, and Tether. To this end, we present the CausalReinforceNet~(CRN) framework, which integrates both Bayesian and dynamic Bayesian network techniques to empower the RL agent in trade decision-making. We develop two agents using the framework based on distinct RL algorithms to analyse performance compared to the Buy-and-Hold benchmark strategy and a baseline RL model. The results indicate that our framework surpasses both models in profitability, highlighting CRN's consistent superiority, although the level of effectiveness varies across different cryptocurrencies.

==> comment.tex <==
% % \documentclass{article}
% % \usepackage{graphicx, xcolor}
% % \usepackage[a4paper, total={6in, 8in}]{geometry}


% \title{Responses to Neurocomputing's Comments on RL Paper}


% % \begin{document}


% \section*{Reviewer 1}
% \begin{enumerate}
%     \item There are several typographical mistakes, such as missing punctuation, that should be corrected with careful reading. \\
%     \textbf{Response:} \textcolor{blue}{Reviewed and corrected as required.}

%     \item One of the most important comments is that you do not provide enough detail about the two Bayesian Networks, as they are presented as black boxes. How does the first Bayesian Network select and process features? (Only Feature Engineering is mentioned, but not enough details). \\
%     \textbf{Response:} \textcolor{blue}{Explanations are added to explain the process of the Bayesian Network in more detail.}

%     \item How does the second (dynamic Bayesian Network) provide predictions? "This process is visually represented by 'Price Direction Prediction with DBN' in Figure 2." This shows only a "black box" with a label. \\
%     \textbf{Response:} \textcolor{blue}{Explanations are added to explain the process of the Dynamic Bayesian Network in more detail.}

%     \item Do these models require any hyperparameters? There should be at least a written explanation and/or an architectural diagram for these BNs. \\
%     \textbf{Response:} \textcolor{blue}{References to BN and DBN papers are now added which should clarify this.}

%     \item Regarding feature selection, provide any explanations for the following: (a) why does the feature selection process yield different feature categories for each altcoin? Also (b) How stable are these results in terms of randomization \\
%     \textbf{Response:} \textcolor{blue}{We need to talk about this.}

%     \item State clearly if both DRL models were used with default hyper-parameters. If yes, provide some justification for this decision. If not, provide details regarding the hyper-parameter tuning process. \\
%     \textbf{Response:} \textcolor{blue}{Explanation is added in the experiment section why we use default settings.}

%     \item How often does the system need retraining to remain competitive? For example, was it retrained with a rolling scheme during the testing period? \\
%     \textbf{Response:} \textcolor{blue}{The frequency of retraining for the system to remain competitive depends on several factors, including market volatility, changes in data patterns, and the model's performance over time. Typically, in fast-changing markets like cryptocurrencies, models might need to be retrained more frequently to adapt to new data.}

%     \item What factors change in the 5 random repetitions of the experiments? (e.g., is it only the random initialization of the models?) \\
%     \textbf{Response:} \textcolor{blue}{Several factors could change across the five random repetitions of the experiments. These include the initialisation of the model and other elements such as the weight of trade positions. These variations contribute to different outcomes in each run, affecting how the agent behaves under varying market conditions.}

%     \item Don't understand the word blue in the following "These probabilities indicate the likelihood or chance of the agent blue performing each possible action" \\
%     \textbf{Response:} \textcolor{blue}{Fixed.}
% \end{enumerate}

% \section*{Reviewer 2}
% \begin{enumerate}
%     \item The methodology presented in the paper exhibits several shortcomings, which are crucial to address for a comprehensive understanding of the study:
%     \begin{itemize}
%         \item Lack of Detailed Explanation for BN and DBN: The paper needs to adequately detail the configuration and operational mechanisms of the Bayesian Network (BN) and Dynamic Bayesian Network (DBN). A clearer exposition of how these networks are structured and function within the scope of the study is essential. \\
%         \textbf{Response:} \textcolor{blue}{Explanations are added to explain the process of BN and DBN in more detail.}

%         \item Ambiguity in Reinforcement Learning Framework: Although the reinforcement learning framework is outlined, the state and action space composition within the study remains unclear. Clarifying these aspects is necessary to fully understand the framework's application. \\
%         \textbf{Response:} \textcolor{blue}{More explanations are added to explain the states and actions.}

%         \item Trading Amount and RL Application: The paper suggests that the trading amount is determined by a rule-based approach rather than learned parameters through Reinforcement Learning (RL). This raises questions about RL's role, which is limited to generating buy, neutral, and sell signals. This aspect seems inconsistent with prior assertions and requires further clarification. \\
%         \textbf{Response:} \textcolor{blue}{More explanation is added in this regard.}

%         \item Lack of Hyperparameter Information and Reproducibility: The absence of detailed hyperparameter settings and the unavailability of code for replication makes the reproducibility of the results uncertain. This omission makes it unlikely for other researchers to validate or build upon the study's findings. \\
%         \textbf{Response:} \textcolor{blue}{We use default parameters. I added justification for this.}

%         \item Inadequate Experimental Evidence and Comparison: The paper lacks sufficient evidence supporting the benefits of using DBN and BN, and no statistical tests seem to have been performed to validate the claims. The comparison is limited to the Buy-and-Hold strategy, neglecting a direct comparison with a standard Proximal Policy Optimization (PPO) approach without BN and DBN. Testing variations that include and exclude DBN and BN would offer a more robust analysis. \\
%         \textbf{Response:} \textcolor{blue}{To address these two comments, I have incorporated an RL base model for each algorithm.}

%         \item Given the daily trading frequency, the training data might need to be increased, potentially leading to overfitting. Exploring higher-frequency data or training across multiple assets could enhance the robustness of the results. Alternatively, using generated data that mimics price distributions might be beneficial. Also, the paper would benefit from a larger dataset with more assets. \\
%         \textbf{Response:} \textcolor{blue}{I added explanations of why we selected this specific time interval.}
%     \end{itemize}
% \end{enumerate}

% % \end{document}

